Men Are Elected, Women Are Married: Events Gender Bias on Wikipedia

Human activities can be seen as sequences of events, which are crucial to understanding societies. Disproportional event distribution for different demographic groups can manifest and amplify social stereotypes, and potentially jeopardize the ability of members in some groups to pursue certain goals. In this paper, we present the first event-centric study of gender biases in a Wikipedia corpus. To facilitate the study, we curate a corpus of career and personal life descriptions with demographic information consisting of 7,854 fragments from 10,412 celebrities. Then we detect events with a state-of-the-art event detection model, calibrate the results using strategically generated templates, and extract events that have asymmetric associations with genders. Our study discovers that the Wikipedia pages tend to intermingle personal life events with professional events for females but not for males, which calls for the awareness of the Wikipedia community to formalize guidelines and train the editors to mind the implicit biases that contributors carry. Our work also lays the foundation for future works on quantifying and discovering event biases at the corpus level.

==> backup/05-related.tex <==
\section{Related Work} \violet{It's fine for a short paper to not have a related work section, as long as you covered the citations in the intro. that can probably save you some space.}
% \paragraph{Faireness in NLP.} 
\paragraph{Faireness in NLP.} NLP researchers have been conducted model-level and corpus-level fairness studies, especially in gender bias. At the model level, ~\citet{Stanovsky2019EvaluatingGB} evaluate the gender bias in machine translation, ~\citet{Zhao2018GenderBI} examine the gender bias in coreference resolution models. At the corpus level, ~\citet{biasemnlp} finds significant gender bias in datasets used for visual recognition 
tasks. There are also other corpus-level fairness studies in addition to gender bias research. For example,  ~\citet{Sap2019TheRO} investigated how annotator's insensitivity to differences in dialect can lead to racial bias in hate speech detection. All the previous works focus on entity analysis. Our work examines the gender bias on events for the first time at the corpus level.

\paragraph{Event Extraction.} Researchers have been paying great attention to event extraction tasks. Neural methods~\cite{Han2019JointEA, lin2020oneie} have shown great improvement compared to conventional machine learning models (e.g., ~\cite{chambers-2013-navytime}). Our work is the first to use the event extraction model as a strength to study bias at the event level.

==> backup/06-conclusion.tex <==
\section{Conclusion and Future Work}
Gender bias of events in career description will potentially lead to discrimination towards females in various professions. In our work, we collected a large-scale career description corpus across 10 occupations from Wikipedia. Via a set of thorough analyses, we found that it is more likely to mix personal life events with career events for females but not for males. To the best of our knowledge, our work is the first to analyze gender bias at the event level. We will make open-source our code and collected dataset together with partially event annotation publicly to facilitate future research. 

Besides the corpus level for events, we also find the event detection model performs differently when we only replace the name placeholder with female or male names during the calibration process, which indicates the potential gender bias at the event detection model level. We will leave this to the future work. Our work is also subject to several limitations. First, it is important to understand and analyze career events for gender minorities (LGBTQ+), missing from our work because of scarce resources online. Future research can build upon our work and go beyond the binary gender, incorporating more experiments on analyzing LGBTQ+ populations' career events. Second, we did not train the event detection model because of the annotation unavailability, so the model may be missing some events. We hope that our work can inspire more researchers to study the fairness for events in general, and introduce more resource to the community. 
